CARD: Controlled Agentic Reddit Discussions for Credit Card Simulation

Online credit card discussions provide a natural setting for studying how consumers communicate about financial products. Simulating these discussions requires more than just generating individual comments, the generated threads should also match how real users express themselves and interact with others. We introduce CARD, a framework for generating realistic credit card discussion threads. Given a credit card post and its matched real thread, CARD uses non-verbatim guidance on reply structure, comment function, stance, tone, and conversational variation. A planner organizes these controls, a writer generates the discussion, and a calibration loop updates comments' populations that contribute to differences between the generated and real thread distributions. We evaluate CARD on real Reddit credit card discussions using lexical, semantic, behavioral, and structural metrics. CARD matches the distributions of real credit card discussions better than simulation baselines across multiple LLMs and also demonstrates smaller effect sizes and distribution distances across metrics. These results show that structured planning and targeted revision can generate the realism of simulated credit card discussions.

==> sections/3-method.tex <==
\section{Methodology}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{framework_v2.png}
    \caption{
    % Overview of CARD. Given a credit card seed post and its matched
    % real thread, The planner models these recurring financial communication behaviors as explicit controls before generation. The writer uses these controls and a partial view of
    % previous comments to generate a new discussion thread. The
    % self-looped reviser then improves the generated collection through
    % four steps: (a) the metric evaluator compares generated and real
    % thread collections across distributional metrics; (b) the
    % controller selects comments that contribute to the current
    % mismatch; (c) the reviser generates best-of-$N$ candidate rewrites;
    % and (d) the metric gate accepts candidates that improve the target
    % metric while preserving protected properties. The revision loop
    % stops when the target metric is no longer significantly different
    % from the real distribution or when the maximum number of
    % iterations is reached.
    Overview of CARD. Given a credit card seed post and its matched
    real discussion, the finance-aware planner represents recurring
    consumer credit card communication behaviors as explicit
    discussion-level and comment-level controls. These controls specify
    how consumers organize replies, address product-specific financial
    issues, express positions on financial claims, and develop
    cost--benefit reasoning. The writer follows these controls and a
    partial view of previous comments to generate a new discussion. The
    self-looped reviser then improves the generated discussion collection
    through four steps: (a) the metric evaluator compares the generated
    and real collections across distributional metrics; (b) the
    controller selects comments that contribute to the current mismatch;
    (c) the reviser generates best-of-$N$ candidate rewrites; and
    (d) the metric gate accepts candidates that improve the target
    metric while preserving protected properties. The revision loop
    stops when the target metric is no longer significantly different
    from the real distribution or when the maximum number of iterations
    is reached.
    }
    \label{fig:framework}
\end{figure*}

% Given a real credit card seed post, CARD generates a new discussion
% that matches how consumers communicate and interact in real credit
% card communities. Given a real credit card seed post, CARD generates a new discussion that matches how consumers communicate and interact in real credit
% card communities. CARD consists of three components: a finance-aware planner, a writer,
% and a metric-guided reviser. The planner constructs an abstract
% thread plan using the matched real discussion as non-verbatim
% guidance. The writer follows the plan to generate a new Reddit-style
% discussion, and the reviser applies iterative edits guided by
% statistical comparisons of thread-level metric distributions. 

Given a credit card seed post, CARD simulates how consumers
interpret, evaluate, and communicate about credit card products in
online discussions. These discussions are organized around
consumer financial decisions. Participants compare rewards and
fees, explain product rules,
% and eligibility constraints, 
evaluate
product value under different spending patterns, qualify or correct
financial claims, and share product-specific experiences.

CARD models three properties of this communication. First, it models
how credit card discussions are organized through reply structures
and recurring communication functions, such as questions,
recommendations, explanations, corrections, and experience sharing.
Second, it models the financial content and reasoning of individual
comments through product-specific issue types, financial claim
stances, and reasoning moves involving benefits, costs, constraints,
and trade-offs. Third, it calibrates population-level communication
patterns so that the generated discussion collection matches those
observed in real credit card communities. CARD implements these
properties through finance-aware communication planning, controlled
comment generation, and distributional calibration.
\subsection{Task Formulation}
CARD represents an online credit card discussion as a discussion
thread rooted at a credit card seed post. We use discussion
to refer to the complete thread, including the seed post, comments,
and reply relations. A post $p$ is the root item that starts a discussion:
$p=(p_{\text{title}},p_{\text{body}}, \allowbreak
p_{\text{prod}},p_{\text{comm}}).$ A comment $c_i$ is a response either to the root post or to another
comment. A discussion thread contains the root post and all
associated comments and reply relations:
\[
T_p =
\left(
p,
\{(c_i,r_i)\}_{i=1}^{n_p}
\right),
\]
where $r_i$ identifies the parent of comment $c_i$, either the root
post or an earlier comment. For a collection of seed posts
$\mathcal{P}$, CARD generates a collection of threads
\(
\hat{\mathcal{T}}
=
\{\hat{T}_p\}_{p\in\mathcal{P}}.
\)

% \noindent The root post is held fixed, which provides the credit card topic and product context for generation, while CARD generates the number of comments, the reply structure, and the text of each comment. CARD targets how credit card discussions are expressed and
% organized, rather than the specific content of a matched real
% thread. 
\noindent The seed post defines the credit card product and discussion context. CARD generates the remaining discussions, including the reply structure, the number of comments, and the text of each comment. The objective is to simulate how consumers communicate about the given credit card product rather than reproduce a particular real discussion.
At the thread level, it controls the number of comments,
reply depth, and branch structure. At the comment level, CARD controls each comment's financial discussion function together with its issue type, reasoning move, stance, tone, length, and opening style.

% Across a collection of threads, CARD aims to match observable communication patterns,
% including lexical and semantic variation, story content,
% disagreement, tone, emotion, comment length, and reply structure. The matched real thread is therefore used only as non-verbatim
% guidance for how the discussion unfolds. 

Across a collection of discussion threads, CARD aims to reproduce the
population-level communication patterns of real credit card
communities, including lexical and semantic variation, disagreement, tone, personal stories, emotion, and discussion thread structure.

\subsection{Distributional Matching Objective}

Let $\phi_k(T_p)$ denote the value of metric $k$ computed for one
discussion thread $T_p$. The metrics cover linguistic, behavioral,
and structural aspects, including lexical repetition, semantic
variation, comment length, reply depth, disagreement, tone, story
content, and emotion. Their full definitions are given in
Section~\ref{sec:evaluation}. For a collection of threads $\mathcal{T}$, define the empirical
metric distribution
\[
\Phi_k(\mathcal{T})
=
\{\phi_k(T):T\in\mathcal{T}\}.
\]
Given a generated thread collection $\hat{\mathcal{T}}$ and its
matched real collection $\mathcal{T}^{\mathrm{real}}$, CARD generates discussion threads that
reduce the discrepancy between
$\Phi_k(\hat{\mathcal{T}})$ and
$\Phi_k(\mathcal{T}^{\mathrm{real}})$
for each metric $k=1,\ldots,K$.

% This objective is defined at the collection level. The matched thread provides abstract guidance over discussion
% structure and communication behavior, while evaluation compares
% metric distributions across the full generated and real
% collections.

\noindent\textbf{Statistical diagnostics.}
We evaluate distributional alignment using the Mann--Whitney U \citep{mann1947test} and Kolmogorov--Smirnov tests \citep{an1933sulla}, together with Cliff's $\delta$ and Wasserstein distance. We use these tests as mismatch diagnostics. We also interpret the test results together
with Cliff's $\delta$ and Wasserstein distance. 

\subsection{Framework Overview}

% Each seed post is paired with its real discussion thread. Let
% $T_p^{\mathrm{real}}$ denote this matched real thread. CARD extracts non-verbatim structural and comment-level controls from
% the matched real thread. 
For each credit card seed post, CARD retrieves one matched real discussion thread about the same financial scenario. The matched discussion thread provides non-verbatim guidance for how consumers communicate, rather than content to reproduce. The overall process is
\[
A_p = P(p,T_p^{\mathrm{real}}),
\qquad
\tilde{T}_p = W(p,A_p),
\qquad
\hat{T}_p =
R\!\left(
\tilde{T}_p,
E(\tilde{T}_p,T_p^{\mathrm{real}})
\right).
\]
Here, $P$ plans the discussion thread, $A_p$ is the abstract thread plan, $W$ generates consumer interactions, and $\tilde{T}_p$ is the initial generated discussion thread. The
evaluator $E$ computes the thread-level metric values used during
calibration, and $R$ calibrates the final collection of discussion threads toward the communication patterns of real credit card communities $\hat{T}_p$. Figure~\ref{fig:framework} presents an overview of the framework.

\subsubsection{\textbf{Discussion planner}}

% The planner decides the structure and communication pattern of the
% thread before natural-language comments are generated. It builds the
% plan at two levels: a thread-level plan and a comment-level plan.

Credit card discussions exhibit recurring financial communication
behaviors that are largely absent from general online discussions.
Consumers recommend products, explain reward rules, qualify
financial claims, compare fees and benefits, and introduce practical
trade-offs. The planner explicitly models these recurring financial
communication behaviors before discussion generation.

\noindent\textbf{Thread level.}
% The planner sets the target number of comments, the number of
% top-level and nested replies, the reply depth, and the branch
% pattern. 

At the discussion thread level, CARD plans how a financial conversation
develops over time by
controlling the number of comments, reply depth, branch structure,
and the balance between top-level and nested replies. These quantities are derived from the matched real thread
and controlled by global generation parameters, such as
comment-count and thread size.

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\caption{Consumer-finance discussion controls used by the CARD
planner.}
\label{tab:planner_controls}
\begin{tabularx}{\columnwidth}
{@{}p{0.07\columnwidth}p{0.34\columnwidth}X@{}}
\toprule
Symbol & Control & Purpose \\
\midrule
$r_i$
& Parent
& Places the comment in the reply tree \\

$d_i$
& Depth
& Controls its structural position \\

$\ell_i$
& Length
& Controls the approximate comment length \\

$f_i$
& Financial discussion function
& Sets the role of the comment in the credit card discussion \\

$s_i$
& Financial claim stance
& Controls support, qualification, or disagreement with a claim \\

$\tau_i$
& Tone
& Controls how the comment is expressed \\

$q_i$
& Financial issue type
& Identifies the aspect of the seed discussion that the comment naturally develops\\

$o_i$
& Opening style
& Reduces repeated comment openings \\

$m_i$
& Financial reasoning move
& Specifies how the comment develops the discussion \\
\bottomrule
\end{tabularx}
\end{table}

\noindent\textbf{Comment level.}
For each planned comment, CARD specifies its communication role
before text generation. The abstract plan is
\[
A_p = \{a_i\}_{i=1}^{\hat{n}},
\]
where $\hat{n}$ is the target number of generated comments. Each
comment plan is represented as
\[
a_i =
\left(
r_i,
d_i,
\ell_i,
f_i,
s_i,
\tau_i,
q_i,
o_i,
m_i
\right).
\]

% The planner variables cover five forms of control: reply structure, discussion composition, interaction style, financial issue coverage, and financial reasoning variation. 
Together, these controls describe how consumers participate in a
credit card discussion thread, including where they reply, what financial
issue they discuss, how they express their position, and how they
develop their reasoning.
The financial issue type $q_i$ specifies what part of the credit
card discussion the comment addresses, while the financial reasoning
move $m_i$ specifies how the comment develops that discussion. For
example, a comment may address product value as its issue type and
introduce a practical trade-off as its reasoning move. These controls
are designed to model the ways in which consumers discuss credit
card products; they do not verify whether the financial statements
made by a generated comment are correct. The variables form a compact control set for the
communication properties that CARD generates and evaluates.
Table~\ref{tab:planner_controls} summarizes each variable.

\begin{cardexample}{Running Example: Planner Output}

\textbf{Thread structure:}
37 comments; 12 top-level replies; 4 subthreads; maximum depth 4.

\smallskip
\textbf{Planned comment:}

\begin{tabularx}{\linewidth}{@{}>{\bfseries}lX@{}}
Function:
& Skeptical correction with a practical caveat. \\

Issue:
& Practical value of the DoorDash credit. \\

Reasoning move:
& Introduce fees and markup as a trade-off. \\

Stance:
& Qualify the parent claim. \\

Tone:
& Casual and skeptical. \\

Opening:
& ``Sure, if you ignore the delivery fees \ldots'' \\
\end{tabularx}

\end{cardexample}

\subsubsection{\textbf{Writer}}

% The writer executes the abstract plan by generating comments
% sequentially. 
The writer generates the discussion thread by one comment at a time while
following the planned communication role of each comment. For the $i$-th comment, the writer produces
\[
c_i
\sim
P_{\theta}
\left(
c_i
\mid
p,
a_i,
c_{r_i},
H_i
\right),
\]
where $a_i$ is the comment plan, $c_{r_i}$ is the generated parent
comment when applicable, and $H_i$ is the visible portion of the
previously generated comments in the same thread.

\noindent The writer receives the seed post, its credit card product context,
the comment plan, the generated parent comment, and selected previous
comments. It then generates a new comment that follows the controls
in $a_i$. Since comments are generated in reply order, later comments
can extend, qualify, correct, question, support, or challenge earlier
comments.

\noindent\textbf{Prompt controls.}
Each field in $a_i$ is converted into an explicit writer instruction.
The writer receives the planned parent relation, target length,
financial discussion function, financial claim stance, tone,
financial issue type, opening style, and financial reasoning move.
These controls specify what role the comment should play and how it
should be expressed, while the model generates new text conditioned
on the seed post and local thread context.

\noindent\textbf{Context dropout and variation.}
% The visible history $H_i$ is varied across comment generations.
Consumers rarely read an entire discussion thread before replying.
CARD therefore varies the visible discussion thread history during
generation. Context dropout removes part of the previously generated thread from
the current writer's view, while context variation changes which
earlier comments are emphasized in the prompt. The seed post and the
direct parent comment remain available as always so that the generated comment
continues to address the current credit card discussion. This design is inspired by dropout in neural network training, where
randomly omitting part of the available representation reduces
co-adaptation and encourages more robust behavior
\citep{srivastava2014dropout}. In CARD, exposing each generated
comment to a partial and slightly different view of the discussion thread
encourages varied responses and reduces repeated semantic patterns.
It also reflects online discussion thread behavior, where participants do
not attend to every earlier comment equally.

\begin{cardexample}{Running Example: Writer Prompt}

\smallskip
Write a comment based on the planned instruction and previous
comments.

\smallskip
\textbf{Planned instruction:}
skeptical correction; casual tone; qualify the parent claim; discuss
the pickup-markup trade-off.

...

\smallskip
\textbf{Visible context:}
[a partial view of earlier comments discussing pickup prices]

\smallskip
\textbf{Writing instructions:}
write a natural Reddit-style reply, do not copy previous comments,
and reply directly to the parent.

\end{cardexample}

\subsubsection{\textbf{Self-Looped Reviser}}

% After the writer generates the initial discussion collection
% $\tilde{\mathcal{T}}$, CARD applies a self-looped revision stage. 
Individual comments may appear realistic while the overall
discussion thread collection still differs from real credit card
communities. CARD therefore applies a self-looped revision stage
to calibrate the collection of discussion threads' communication patterns. 
The reviser improves one target metric at a time while treating all other
metrics as protected metrics. The reviser also preserves the local discussion thread plan, including the
seed post, reply tree, planned financial discussion function,
financial claim stance, financial issue type, reasoning move, and
reply target. These checks preserve the intended communication role
of the comment. The revision loop continues
until neither statistical test detects a significant difference for
the target metric or the maximum number of revision iterations reached.

\noindent\textbf{Round diagnosis and protection policy.}
Each revision round starts by comparing the current generated
collection with the matched real collection using the metric families
in Section~\ref{sec:evaluation}. If statistical tests detect a
significant difference between the generated and real distributions
for a metric, the controller selects that metric as the target metric
$\phi_t$. All other metrics form the protected set
\[
\mathcal{P}_t
=
\mathcal{M}\setminus\{\phi_t\}.
\]
The round is allowed to reduce the mismatch in $\phi_t$, while the
metrics in $\mathcal{P}_t$ must remain within tolerance. The
controller also identifies where the generated--real gap occurs,
such as the upper tail or middle mass, and selects the revision
operations for the round.

\begin{cardexample}{Running Example: Round Diagnosis}

\begin{tabularx}{\linewidth}{@{}Xr@{}}
\textbf{Metric} & \textbf{Result} \\
\hline
Self-BLEU
& \textcolor{red}{\xmark} \\

Semantic cosine similarity
& \textcolor{green!60!black}{\cmark} \\

Disagreement rate
& \textcolor{green!60!black}{\cmark} \\

Politeness rate
& \textcolor{green!60!black}{\cmark} \\

Comment length
& \textcolor{green!60!black}{\cmark} \\

Comment depth
& \textcolor{green!60!black}{\cmark} \\

Emotion entropy
& \textcolor{green!60!black}{\cmark} \\
\end{tabularx}

\smallskip
\textbf{Target metric:} Self-BLEU.

\textbf{Protected metrics:} All remaining metrics.

\end{cardexample}

\noindent\textbf{Thread and comment selection.}
Given a target metric $\phi_t$, CARD first computes a target-metric
gap for each generated thread. For a generated thread $T_p$ and its
matched real thread $T_p^{\mathrm{real}}$, the gap is
\[
g_t(T_p)
=
\left|
\phi_t(T_p)
-
\phi_t(T_p^{\mathrm{real}})
\right|.
\]
Threads with larger $g_t(T_p)$ are selected first because they
contribute more to the current mismatch. Within each selected thread, CARD ranks comments by how strongly they
contribute to the target metric. For example, in Self-BLEU, comment contribution
is estimated from within-thread lexical overlap. CARD compares the
target comment with other comments in the same thread, counts shared
repeated $n$-grams, and detects repeated opener and connector
patterns. Comments with larger overlap scores are revised first.

\begin{cardexample}{Running Example: Thread and Comment Selection}

\textcolor{green!60!black}{\cmark}\;
\emph{Is the DoorDash credit basically just \$5 off after fees and
markup?}

\smallskip
\textcolor{green!60!black}{\cmark}\;
\emph{Existing DoorDash users only.}

\smallskip
\textcolor{red}{\xmark}\;
\emph{Thanks, yeah, pickup usually stretches it further. I'd stick
to low-markup spots.}

\smallskip
\textcolor{green!60!black}{\cmark}\;
\emph{Just a clearing delay, not a card glitch.}

\smallskip
The third comment is selected because it contributes most to the
Self-BLEU mismatch.

\end{cardexample}

\noindent\textbf{Candidate generation.}
For each selected comment, CARD first samples candidate rewrites
using a predefined set of metric-specific revision operations. The
controller selects these operations based on the current target
metric and the detected failure pattern. If the predefined operations do not produce an effective revision,
the controller asks an LLM to generate additional revision
instructions. These instructions are conditioned on the current
failure pattern and the revision history, including previously used
instructions and their outcomes. This allows the controller to avoid
repeating ineffective edits and to propose a more targeted revision
strategy for the current comment. If the controller selects $K$ operations and samples N candidates for each operation, CARD evaluates $K \times N$ candidate rewrites for that comment:
\[
\mathcal{C}_i
=
\left\{
c_i^{\prime(k,n)}
\right\}_{k=1,n=1}^{K,N}.
\]
The candidate prompt includes the target comment, its parent comment,
selected earlier comments, and the planned financial discussion
function, claim stance, issue type, and reasoning move.

\begin{cardexample}{Running Example: Candidate Generation}

\textbf{Target comment:}

\emph{Thanks, yeah, pickup usually stretches it further. I'd stick
to low-markup spots.}

\smallskip
\textbf{1. Revise opener}

\begin{enumerate}
    \setlength{\itemsep}{1pt}
    \setlength{\topsep}{2pt}
    \item \emph{Yeah, pickup usually costs more. I'd stick to
    low-markup spots.}
    \item \emph{True, pickup tends to add more. I'd choose
    low-markup places.}
    % \item \emph{Agreed, pickup often pushes it higher. I'd avoid
    % high-markup spots.}
\end{enumerate}

\textbf{2. Change wording}

\begin{enumerate}
    \setlength{\itemsep}{1pt}
    \setlength{\topsep}{2pt}
    \item \emph{Pickup usually adds even more. I'd go with
    low-markup places.}
    \item \emph{Pickup tends to raise the price further. I'd keep
    to cheaper spots.}
    % \item \emph{Pickup often increases the total. I'd choose places
    % with smaller markups.}
\end{enumerate}

\textbf{3. Merge sentences}

\begin{enumerate}
    \setlength{\itemsep}{1pt}
    \setlength{\topsep}{2pt}
    \item \emph{Since pickup usually costs more, I'd stick to
    low-markup spots.}
    \item \emph{Because pickup adds more, I'd choose low-markup
    places.}
    % \item \emph{Pickup tends to push prices up, so I'd avoid
    % high-markup spots.}
\end{enumerate}

\end{cardexample}

\noindent\textbf{Candidate scoring and acceptance.}
For each candidate rewrite $c_i'\in\mathcal{C}_i$, CARD forms a
candidate thread $T_i'$ by replacing only $c_i$ with $c_i'$. The
candidate receives a target-gap reduction score:
\[
R_t(c_i')
=
g_t(T^{(m)})
-
g_t(T_i'),
\]
where $T^{(m)}$ is the current thread before the edit. A positive
$R_t(c_i')$ means that the candidate moves the thread closer to its
matched real thread on the target metric. A candidate is valid when
\[
R_t(c_i')>\epsilon_t,
\qquad
\operatorname{Preserve}(a_i,c_i')=1.
\]
The preservation check requires the rewrite to retain the planned
financial discussion function, financial claim stance, financial
issue type, reasoning move, approximate length, and reply target.
This check preserves the planned communication behavior of the
comment. 
% ; it does not evaluate the correctness of its financial claims

CARD may also apply metric-specific local gates. For example, the
Self-BLEU reviser checks whether the rewritten comment reduces its
lexical overlap with other comments in the same thread. Among valid
candidates, CARD selects the candidate with the largest
$R_t(c_i')$. If no candidate satisfies the acceptance conditions,
the original comment is left unchanged.

\begin{cardexample}{Running Example: Candidate Acceptance}

\begin{minipage}[t]{0.47\linewidth}
\textbf{Candidate 1}

\smallskip
\emph{Yeah, pickup is still expensive. Use cheaper places.}

\smallskip
\textcolor{red}{\xmark}\; Self-BLEU

\textcolor{red}{\xmark}\; Semantic cosine

\textcolor{green!60!black}{\cmark}\; Disagreement

\textcolor{green!60!black}{\cmark}\; Politeness

\textcolor{green!60!black}{\cmark}\; Length

\textcolor{red}{\xmark}\; Emotion

\smallskip
\textbf{Rejected}
\end{minipage}
\hfill
\begin{minipage}[t]{0.47\linewidth}
\textbf{Candidate 2}

\smallskip
\emph{Since pickup often raises the price, I'd stick to restaurants
with low markups.}

\smallskip
\textcolor{green!60!black}{\cmark}\; Self-BLEU

\textcolor{green!60!black}{\cmark}\; Semantic cosine

\textcolor{green!60!black}{\cmark}\; Disagreement

\textcolor{green!60!black}{\cmark}\; Politeness

\textcolor{green!60!black}{\cmark}\; Length

\textcolor{green!60!black}{\cmark}\; Emotion

\smallskip
\textbf{Accepted}
\end{minipage}

\end{cardexample}

\noindent\textbf{Applying candidate edits.}
Each accepted rewrite replaces the original comment at the same
position in its thread. The root post, parent relation, and all
unrevised comments remain unchanged. After all selected comments
have been processed, the updated threads form a proposed thread
collection for the current round:
\(
\hat{\mathcal{T}}_{\mathrm{prop}}^{(r+1)}.
\)
CARD then recomputes every evaluation metric over the complete
proposed collection. Local candidate scores therefore determine
which edits are proposed, while collection-level statistics
determine whether the entire revision round is retained.

\noindent\textbf{Round-level acceptance and rollback.}
CARD maintains the most recent accepted thread collection
$\hat{\mathcal{T}}^{(r)}$. In round $r+1$, the reviser produces a
proposed collection
$\hat{\mathcal{T}}_{\mathrm{prop}}^{(r+1)}$. CARD then rescores the
complete proposed collection and compares its metric quality with
that of the most recent accepted collection.The proposed round is accepted only if it improves the target metric
and does not cause any protected metric to degrade beyond its
configured tolerance. If accepted, the proposed collection becomes
the input to the next round; otherwise, CARD rolls back to the most
recent accepted collection:
\[
\hat{\mathcal{T}}^{(r+1)}
=
\begin{cases}
\hat{\mathcal{T}}_{\mathrm{prop}}^{(r+1)},
& \text{if the round is accepted},\\
\hat{\mathcal{T}}^{(r)},
& \text{otherwise}.
\end{cases}
\]
When the revision process stops, CARD returns the most recent
accepted collection.

\begin{table*}[!t]
\centering
\footnotesize
\setlength{\tabcolsep}{1.45pt}
\renewcommand{\arraystretch}{1.10}

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}ll*{12}{cc}c@{}}
\toprule

\multirow{2}{*}{Method}
& \multicolumn{1}{c}{\multirow{2}{*}{Model}}
& \multicolumn{2}{c}{Self-BLEU}
& \multicolumn{2}{c}{Self-BERT}
& \multicolumn{2}{c}{Sem. Cos.}
& \multicolumn{2}{c}{Hard Dis.}
& \multicolumn{2}{c}{Polite}
& \multicolumn{2}{c}{Impolite}
& \multicolumn{2}{c}{Neutral}
& \multicolumn{2}{c}{Len. CV}
& \multicolumn{2}{c}{Depth}
& \multicolumn{2}{c}{Virality}
& \multicolumn{2}{c}{Story}
& \multicolumn{2}{c}{Emotion}
& \multirow{2}{*}{\makecell{Non-rej.\\(\%)}} \\

\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
\cmidrule(lr){15-16}
\cmidrule(lr){17-18}
\cmidrule(lr){19-20}
\cmidrule(lr){21-22}
\cmidrule(lr){23-24}
\cmidrule(lr){25-26}

& & MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& MWU & KS
& \\

\midrule

\multirow{4}{*}{OASIS}
& gemini-2.5-flash
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.0 \\

& deepseek-v4-flash
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.037 & \textbf{0.073}
& 4.2 \\

& gpt-4o-mini
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.001 & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.048 & \textbf{0.053}
& 4.2 \\

& gpt-5.4-mini
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.039 & 0.020
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.0 \\
\midrule

\multirow{4}{*}{SynthPAI}
& gemini-2.5-flash
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& \textbf{0.186} & \textbf{0.073}
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& \textbf{0.054} & \textbf{0.098}
& $<\!0.001$ & $<\!0.001$
& \textbf{0.102} & 0.004
& \textbf{0.197} & 0.013
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 25.0 \\

& deepseek-v4-flash
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.034 & \textbf{0.169}
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& \textbf{0.495} & \textbf{0.129}
& \textbf{0.868} & \textbf{0.073}
& \textbf{0.581} & \textbf{0.073}
& \textbf{0.260} & \textbf{0.073}
& $<\!0.001$ & $<\!0.001$
& 37.5 \\

& gpt-4o-mini
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & 0.006
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& \textbf{0.896} & \textbf{0.073}
& \textbf{0.881} & 0.039
& $<\!0.001$ & $<\!0.001$
& \textbf{0.731} & \textbf{0.129}
& 20.8 \\

& gpt-5.4-mini
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& \textbf{0.858} & \textbf{0.276}
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 0.002 & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& $<\!0.001$ & $<\!0.001$
& 8.3 \\

\midrule

\multirow{4}{*}{\textbf{CARD}}
& gemini-2.5-flash
& \textbf{0.159} & \textbf{0.059}
& $<\!0.001$ & $<\!0.001$
& \textbf{0.917} & \textbf{0.443}
& \textbf{0.233} & \textbf{0.058}
& \textbf{0.508} & \textbf{0.725}
& $<\!0.001$ & $<\!0.001$
& \textbf{0.361} & \textbf{0.532}
& \textbf{0.392} & \textbf{0.817}
& \textbf{0.094} & \textbf{0.291}
& \textbf{0.053} & \textbf{0.291}
& \textbf{0.979} & \textbf{0.984}
& \textbf{0.063} & \textbf{0.180}
& \textbf{83.3} \\

& deepseek-v4-flash
& \textbf{0.381} & \textbf{0.106}
& \textbf{0.973} & \textbf{0.725}
& \textbf{0.266} & \textbf{0.443}
& \textbf{0.458} & \textbf{0.725}
& \textbf{0.245} & \textbf{0.817}
& \textbf{0.489} & \textbf{0.817}
& \textbf{0.805} & \textbf{0.951}
& \textbf{0.537} & \textbf{0.628}
& \textbf{0.580} & \textbf{0.951}
& \textbf{0.452} & \textbf{0.894}
& 0.019 & 0.011
& \textbf{0.792} & \textbf{0.725}
& \textbf{91.7} \\

& gpt-4o-mini
& 0.020 & 0.011
& $<\!0.001$ & $<\!0.001$
& 0.014 & 0.015
& 0.024 & 0.001
& \textbf{0.344} & \textbf{0.231}
& \textbf{0.081} & \textbf{0.231}
& 0.003 & 0.022
& 0.028 & 0.005
& \textbf{0.079} & \textbf{0.180}
& \textbf{0.057} & \textbf{0.139}
& \textbf{0.149} & \textbf{0.291}
& $<\!0.001$ & $<\!0.001$
& \textbf{41.7} \\

& gpt-5.4-mini
& \textbf{0.307} & \textbf{0.139}
& \textbf{0.323} & \textbf{0.362}
& \textbf{0.373} & \textbf{0.532}
& \textbf{0.848} & \textbf{0.997}
& 0.006 & 0.031
& \textbf{0.770} & \textbf{0.997}
& \textbf{0.185} & \textbf{0.725}
& \textbf{0.393} & \textbf{0.291}
& \textbf{0.258} & \textbf{0.816}
& \textbf{0.134} & \textbf{0.532}
& \textbf{0.260} & \textbf{0.291}
& \textbf{0.892} & \textbf{0.816}
& \textbf{91.7} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Metric-level statistical comparison across methods and models. Each metric reports Mann--Whitney U and Kolmogorov--Smirnov $p$-values. Values with $p>0.05$ are bolded, indicating that the corresponding test does not detect a statistically significant difference between the generated and real distributions. Non-rej. (\%) reports the percentage of metric--test pairs for which
the null hypothesis is not rejected at $\alpha=0.05$ for all 12 metrics.
}
\label{tab:pvalue_results}
\end{table*}
